Mechanisms for Outsourcing Computation via a Decentralized Market

As the number of personal computing and IoT devices grows rapidly, so does the amount of computational power that is available at the edge. Since many of these devices are often idle, there is a vast amount of computational power that is currently untapped, and which could be used for outsourcing computation. Existing solutions for harnessing this power, such as volunteer computing (e.g., BOINC), are centralized platforms in which a single organization or company can control participation and pricing. By contrast, an open market of computational resources, where resource owners and resource users trade directly with each other, could lead to greater participation and more competitive pricing. To provide an open market, we introduce MODiCuM, a decentralized system for outsourcing computation. MODiCuM deters participants from misbehaving-which is a key problem in decentralized systems-by resolving disputes via dedicated mediators and by imposing enforceable fines. However, unlike other decentralized outsourcing solutions, MODiCuM minimizes computational overhead since it does not require global trust in mediation results. We provide analytical results proving that MODiCuM can deter misbehavior, and we evaluate the overhead of MODiCuM using experimental results based on an implementation of our platform.

==> analysis.tex <==
\section{Analysis of \platform Incentives}


While the trustworthy execution of the Smart Contract can ensure the correctness of the participants' interactions with the platform, it cannot prevent misbehavior, such as posting incorrect jobs or results on a Directory (see Section~\ref{subsec:misbehavior}).
Since verification and mediation cannot always detect and punish misbehavior, the fines and rewards must deter misbehavior and incentivize participants to act honestly and comply with the workflow.
In this section, we show using game theory that selfish rational actors will indeed choose to act honestly\Aron{when! parameters!}.

\subsection{Actors and Strategies}
Since our computation market is open and decentralized, RPs and JCs may join or leave the platform or create new identities at any time.
Consequently, we have to show that RPs and JCs are incentivized to act honestly in every single interaction.
By a single interaction, we mean a single execution of the workflow starting from uploading the job and posting the resource and job offers.
%We prove that once a resource and job offer are matched, the RP and JC will make their best effort to execute the job and follow the workflow correctly.
We model this interaction as a \emph{two-player non-cooperative game} between an RP and a JC.

Note that we assume Directories and Mediators  always act honestly, so we do not consider their strategic decisions in our analysis.
The rationale behind this assumption is that RPs and JCs can choose which Directories and Mediators they trust; hence, they will quickly blacklist the ones that misbehave.
Since the business model for Directories and Mediators is attracting RPs and JCs who trust and pay them for their services, they have very strong incentives to build a positive reputation in the ecosystem. The formal proof for this conjecture will be provided in future work.\taha{Not included in the future work.}


The JC can choose from two strategies:
%\begin{description}
%\item 
\emph{Comply} ($Cj$), which models the JC making its best effort to follow the workflow correctly; %  JC uses the system as intended in good faith.
%\item 
and \emph{Disobey} ($Dj$), which models the JC trying to ``cheat'' by uploading an incorrect job but claiming it to be correct, rejecting a job result even if it is correct, claiming that the RP did not post a result, etc. (see Section~\ref{subsec:misbehavior}). % that job results that the   JC claims that RP submitted an incorrect solution. (This will encompass the strategy of JC claiming that RP submitted no solution. Since verifying a solution is more expensive than checking if the solution exists, especially since the RP's solution will be posted on the ledger and should be trivial to check.

Similarly, the RP can choose from two strategies:
%\begin{description}
%\item 
\emph{Comply} ($Cr$), which models the RP making its best effort to follow the workflow correctly (note that the RP may fail due to reliability failure, but this is not considered malicious behavior); % Resource Provider uses the system as intended in good faith. All mistakes are unintentional and rare.
%\item 
and \emph{Disobey} ($Dr$), which models the RP trying to ``cheat'' by submitting an incorrect (e.g., randomly generated) result for a job, claiming that the job was not uploaded, etc.  %Resource Provider intentionally submits incorrect/random solutions instead of correctly computing jobs.
%\end{description}

\subsection{Notation}

We introduce the following notation for our analysis (see Section~\ref{sec:workflow} for a detailed description of the workflow):
\begin{itemize}[topsep=0pt, noitemsep]

\item $C$: cost incurred by RP for correctly running the job; %, with strategy Cr

\item $C_d$: cost incurred by RP for incorrectly running the job (for strategy $Dr$);  %= computational cost to RP to incorrectly run job, with strategy Dr, $cd >= c$
%\item FR = platform wide fine rate, f = FR * r

\item $Q$: probability that RP manages to correctly run the job, i.e., not suffering any reliability failures (for strategy $Cr$); %faithfully and successfully calculating job result, including the possibility  disruption due to physical and connection issues, $q \in (0,1)$

\item $p$: probability that JC verifies the result;

\item $C_j$: cost incurred by JC for verifying the job result; %, $cj <= c$

\item $M$: cost of mediation by mediator (paid by party at fault) 

\item $P_j$: probability that JC detects incorrect job result via verification; %that the job result  spots error (true positive), false positive rate is 0. 

\item $P_m$: probability that Mediator correctly identifies the misbehaving party ($P_m \geq 0.75$, see Section~\ref{subsec:verification}); % spots error (true positive), false positive rate is 0

\item $r$: reward paid by JC to RP for completing the job (see Equation~\eqref{eq:job_price}); %either unverified job or completion of a successfully verified job %, $r>c$

\item $B$: JC's benefit from receiving the  correct job result;

\item $f$: fine imposed on misbehaving participant (RP or JC).
%f is a multiple of r 

\end{itemize}


\begin{comment}
\subsection{Model}

\Aron{This has already been described in the workflow section, so let's keep it very short. We just need to remind the reader how it works. Maybe a simple section reference will suffice.}

\begin{enumerate}

\item  JC submits job and the deposit.

\item  RP submits resource offer and deposit.

\item  Job offer and resource offer are matched according to contract specifications with Hopcroft-Karp with a singular solver.

\ad{We should clarify that the offers are matched by one solver. }

\item  RP receives job and computes the result, this is where the "game" between the RP and JC begins.

\item  RP posts results.

\item  With P probability, the results are verified by the JC at random.

\item  If the result is verified and approved or if job was not verified, RP earns r reward.

\item  If the result is verified and not approved by the JC, then the Mediator is invoked. The Mediator determines which party is lying. The guilty party is then fined f from the deposit.

\item The remaining deposits are returned.
\end{enumerate}
\end{comment}




\subsection{Utilities}

Next, we express the actors' utilities in the four possible strategy profiles using the above notation.
%For ease of presentation, we introduce two symbols $Z_c$ and $Z_d$.

% $$Z_c = (1-Q) \cdot p \cdot P_j \cdot P_m ,$$ 
%which corresponds to probability of no reward payout assuming cooperative strategy;
%$$Z_d = p \cdot P_j \cdot P_m ,$$ 
%which corresponds to probability of no reward payout assuming a deceptive strategy.

\newcommand{\Util}[1]{\ensuremath{\mathcal{U}_{#1}}}

\textit{Case 1)} Both act honestly $(C_j, C_r)$:

The JC's expected utility is
\begin{align*}
\Util{JC}(C_j, C_r) = 
Q \cdot (B - r) % computation benefit - payout reward
+ (1 - Q) \cdot f %verification and fine/reward
- p \cdot  C_j . % cost of verification
\end{align*}
The first term is the JC's net benefit in case the RP successfully executes the job;
the second term is the fine paid by RP in case of reliability failure;
and the third term is the cost incurred by the JC for verification.

The RP's expected utility is
\begin{align*}
\Util{RP}(C_j, C_r) =
Q \cdot r   %probability of getting paid 
- (1 - Q) \cdot (f + M)  %probability of getting fined, 
- C  .%compute
\end{align*}
The first term is the RP's reward for successfully executing the job;
the second term is the fine paid in case of a reliability failure;
and the third term is the cost of executing the job.

\textit{Case 2)} JC acts honestly, but RP tries to ``cheat'' $(C_j, D_r)$:
\begin{align*}
\Util{JC}(C_j, D_r) =
-(1 - p \cdot P_j) \cdot r
+ p \cdot P_j \cdot f
- p \cdot C_j . 
\end{align*}
The first two terms are job reward and fine in case of missing the RP's misbehavior and in case of detecting it, respectively.
%
\begin{align*}
\Util{RP}(C_j, D_r) = 
(1 - p \cdot P_j) \cdot r % reward
- p \cdot P_j \cdot (f + M) % fine
-C_d . %compuation cost of deceptive strategy
\end{align*}
The first two terms are again the reward received and fine paid. %in case of avoiding detection and getting caught, respectively.

\textit{Case 3)} JC tries to ``cheat,'' but RP acts honestly $(D_j, C_r)$:
\begin{align*}
\Util{JC}(D_j, C_r) = & \hphantom{+}
Q \cdot \left( B %Probability of getting job benefit
+ (1 - P_m) \cdot f
- P_m \cdot (f + M + r) \right) \nonumber \\ %probability of paying reward and fine
& + (1 - Q) \cdot f .
\end{align*}
The first term considers the RP successfully executing the job, which includes: JC's benefit from the result; fine paid by the RP to the JC if the JC manages to deceive the Mediator (note that the best option for this is posting a non-deterministic job, which can result in $P_m \geq 0.75$, see Section~\ref{subsec:verification});
and fine and reward paid by the JC if it fails to deceive the Mediator.
%
\begin{align*}
\Util{RP}(D_j, C_r) = & \hphantom{-}
Q \cdot (P_m \cdot (f + r) - (1 - P_m) \cdot (f + M) \nonumber \\
& - (1 - Q) \cdot (f + M) - C
\end{align*}

\textit{Case 4)} Both actors try to ``cheat'' $(D_j, D_r)$:
%
\begin{align*}
\Util{JC}(D_j, D_r) &= 
(1 - P_m) \cdot f - P_m \cdot (f + M + r)  \\
\Util{RP}(D_j, D_r) &= 
P_m \cdot (f + r) - (1 - P_m) \cdot (f + M) 
-C_d %always do computation
\end{align*}

\subsection{Equilibrium Analysis}

Our goal is to characterize when neither actors have an incentive to act dishonest.
We capture this using the concept of Nash equilibrium.
Formally, strategy profile $(Cj, Cr)$ is a Nash equilibrium if neither actor can increase its own expected utility by unilaterally changing its strategy choice.

\begin{theorem}
\label{thm:NE}
Both RP and JC acting honestly is a Nash equilibrium if and only if
\begin{equation*}
   p  
    \leq 
    Q \frac{P_m \cdot (2 f + M + r) - r -f  }{ C_j}
\end{equation*}
and
\begin{equation*}
 p \geq \frac{(1 - Q)}{P_j} + \frac{C - C_d}{P_j \cdot (r + f + M)} .
\end{equation*}
\end{theorem}

Due to space limitations, we present the proof of Theorem~\ref{thm:NE} in the online appendix on GitHub~\cite{modicum}.

\begin{comment}
\begin{IEEEproof}
First, JC will act honestly if and only if
\begin{align*}
    \Util{JC}(C_j, C_r) &\geq \Util{JC}(D_j, C_r) \\
    Q \cdot (B - r) + (1 - Q) \cdot f \\ - p \cdot  C_j 
    &\geq 
    Q \cdot \big[ B + (1 - P_m) \cdot f \\ &\hphantom{\geq} - P_m \cdot (f + M + r) \big] + (1 - Q) \cdot f .
    \end{align*}
Equivalently,
    \begin{align*}
    - p \cdot  C_j 
    &\geq 
    Q \cdot \big[ r + (1 - P_m) \cdot f  - P_m \cdot (f + M + r) \big] \\
     p  
    &\leq 
    Q \frac{P_m \cdot (f + M + r) - r - (1 - P_m) \cdot f}{ C_j} \\
     p  
    &\leq 
    Q \frac{P_m \cdot (2 f + M + r) - r -f  }{ C_j} .
\end{align*}

Second, the RP will act honestly if and only if
\begin{align*}
    \Util{RP}(C_j, C_r) &\geq \Util{RP}(C_j, D_r) \\
    Q \cdot r - (1 - Q) \cdot (f + M) - C 
    &\geq (1 - p \cdot P_j) \cdot r - p \cdot P_j \cdot (f + M) - C_d .
\end{align*}
Equivalently,
\begin{align*}
 p \cdot P_j \cdot (r +  f + M)
    &\geq (1 - Q) \cdot (f + M + r) + C - C_d \\ 
 p &\geq \frac{(1 - Q) \cdot (f + M + r) + C - C_d}{P_j \cdot (r + f + M)}  \\
 p &\geq \frac{(1 - Q)}{P_j} + \frac{C - C_d}{P_j \cdot (r + f + M)}.
\end{align*}
\end{IEEEproof}
\end{comment}




\begin{comment}
\subsection{Function Inequalities}

\subsubsection{JC Constraints}\hfill

For $\Util{JC}(C_j, C_j)  > 0$ : (to make profit)

For $\Util{JC}(D_j,C_r) < \Util{JC}(C_j,C_r)$:

%For $\Util{JC}(D_j,D_r) < \Util{JC}(C_j,D_r)$:

\subsubsection{RP Constraints}\hfill

For $\Util{RP}(C_j,C_r) > 0$:

for $\Util{RP}(C_j, D_r) < \Util{RP}(C_j, C_r)$:

%for $\Util{RP}(D_j, D_r) < \Util{RP}(D_j, C_r)$:

%insert graphs

\end{comment}



\pgfplotsset{%
  utilaxis/.style={%
    width=0.53\columnwidth,
    height=0.45\columnwidth,
    font=\scriptsize,
    grid=major},
  JCutilaxis/.style={%
    utilaxis,
    ylabel={JC's utility $\Util{JC}$}
  },
  RPutilaxis/.style={%
    utilaxis,
    ylabel={RP's utility $\Util{RP}$}
  },
  eqline/.style={%
    solid,
    blue,
    ultra thick
  },
  noeqline/.style={%
    solid,
    red,
    ultra thick
  }}

\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
      JCutilaxis,
      xlabel={Verification probability $p$}
      ]
      \addplot[noeqline] table[col sep=comma, x index=0, y index=1] {graphs/ProbabilityNoEq.csv};
      \addplot[eqline] table[col sep=comma, x index=0, y index=1] {graphs/ProbabilityEq.csv};
    \end{axis}
    \end{tikzpicture}
    \begin{tikzpicture}
    \begin{axis}[
      RPutilaxis,
      xlabel={Verification probability $p$},
      ]
      \addplot[noeqline] table[col sep=comma, x index=0, y index=2] {graphs/ProbabilityNoEq.csv};
      \addplot[eqline] table[col sep=comma, x index=0, y index=2] {graphs/ProbabilityEq.csv};
    \end{axis}
    \end{tikzpicture}    
    \begin{tikzpicture}
    \begin{axis}[
      JCutilaxis,
      xlabel={Fine $f$}
      ]
      \addplot[noeqline] table[col sep=comma, x index=0, y index=1] {graphs/FineNoEq.csv};
      \addplot[eqline] table[col sep=comma, x index=0, y index=1] {graphs/FineEq.csv};
    \end{axis}
    \end{tikzpicture}
    \begin{tikzpicture}
    \begin{axis}[
      RPutilaxis,
      xlabel={Fine $f$}
      ]
      \addplot[noeqline] table[col sep=comma, x index=0, y index=2] {graphs/FineNoEq.csv};
      \addplot[eqline] table[col sep=comma, x index=0, y index=2] {graphs/FineEq.csv};
    \end{axis}
    \end{tikzpicture}
    \begin{tikzpicture}
    \begin{axis}[
      JCutilaxis,
      xlabel={$P_j = P_m$}
      ]
      \addplot[noeqline] table[col sep=comma, x index=0, y index=1] {graphs/DetectionNoEq.csv};
      \addplot[eqline] table[col sep=comma, x index=0, y index=1] {graphs/DetectionEq.csv};
    \end{axis}
    \end{tikzpicture}
    \begin{tikzpicture}
    \begin{axis}[
      RPutilaxis,
      xlabel={$P_j = P_m$}
      ]
      \addplot[noeqline] table[col sep=comma, x index=0, y index=2] {graphs/DetectionNoEq.csv};
      \addplot[eqline] table[col sep=comma, x index=0, y index=2] {graphs/DetectionEq.csv};
    \end{axis}
    \end{tikzpicture}
    \caption{Job Creator's and Resource Provider's expected utilities when both act honestly (i.e., $(C_j, C_r)$) for various parameter values. Blue segments correspond to values where $(C_j, C_r)$ is an equilibrium, while red segments correspond to value where it is not.}
    \label{fig:utilities}
\end{figure}

\subsection{Numerical Example}
%\subsubsection{Values}

Next, we present a numerical example showing the existence of equilibria where both RP and JC act honestly.
For these examples, unless stated otherwise, we use the following values:
%\begin{description}
%  \begin{minipage}[t]{0.25\textwidth}  
%\item 
$p = 0.1$, 
%\item 
$C = 1$,
%\item 
$r= 1.5 > C$,
%\item 
$f = 100 \cdot r = 150$,
%\item 
$B = 2$,
%\item 
$C_d = 0.1$,
%    \end{minipage}\begin{minipage}[t]{0.25\textwidth} 
%\item 
$C_j = C = 1$,
%\item 
$M = C \cdot 3$,
%\item 
$P_j = 0.999$,
%\item 
$P_m = 0.75$,
%\item
$Q = 0.999$.
%\item $Z_c = 0.00081$
%\item $Z_d = 0.081$
%    \end{minipage}
%\end{description}
Table~\ref{tab:exputil} shows the RP's and JC's expected utilities for the four strategy profiles. Clearly, $(C_j, C_r)$ is a Nash equilibrium.


\begin{table}[h]
\centering
\caption{Expected Utility}
\vspace{-0.8em}
\label{tab:exputil}
\begin{tabular}{|l|l|l|}
\hline
$\Util{JC}, \Util{RP}$ & $C_r$   & $D_r$ \\ \hline
$C_j$ & \textbf{0.550, 0.349}  & 13.535, -13.735    \\ \hline
$D_j$ & -73.901, 74.899  & -76.125, 76.025    \\ \hline
\end{tabular}
\end{table}



Figure~\ref{fig:utilities} shows the JC's and RP's expected utilities when  both act honestly (i.e., $(C_j, C_r)$) for various parameter values.
As predicted by our analysis, both acting honestly is a Nash equilibrium for wide ranges of parameter values.

%\includegraphics[width=\textwidth/2]{UtilityCC.png}

%\includegraphics[width=\textwidth/2]{UtiliyCClabels.png}

==> data/gas/gas_sci.tex <==
Function,mean,std.dev.,gasEstimate
setPenaltyRate,4.34E+04,0.00E+00,2.21E+04
setReactionDeadline,4.31E+04,0.00E+00,2.16E+04
acceptResult,1.40E+05,6.47E+04,6.29E+04
postResult,1.91E+05,1.60E+04,2.25E+05
postMatch,1.35E+05,1.70E+03,1.27E+05
postJobOfferPartOne,2.36E+05,4.59E+03,2.28E+05
postJobOfferPartTwo,2.16E+05,0.00E+00,2.27E+05
postResOffer,2.42E+05,2.16E+03,2.32E+05
registerMediator,1.37E+05,0.00E+00,8.51E+04
registerResourceProvider,8.12E+04,0.00E+00,2.54E+04
resourceProviderAddTM,6.50E+04,0.00E+00,4.23E+04
registerJobCreator,3.40E+04,0.00E+00,3.20E+03
jobCreatorAddTM,6.53E+04,0.00E+00,4.26E+04
postMediationResult,1.87E+05,1.56E+04,2.40E+05
rejectResult,5.39E+04,9.90E+00,4.71E+04
nominal cost, 5.92E+05,,

==> figures/setup-fig.tex <==
\catcode`\_=12 % category other
\pgfplotstableread[col sep=comma]{data/functions_general/jobCreatorAddTrustedMediator.csv}\dtJCATM
\pgfplotstableread[col sep=comma]{data/functions_general/registerJobCreator.csv}\dtRegJC
\pgfplotstableread[col sep=comma]{data/functions_general/registerMediator.csv}\dtRegM
\pgfplotstableread[col sep=comma]{data/functions_general/registerResourceProvider.csv}\dtRegRP
\pgfplotstableread[col sep=comma]{data/functions_general/resourceProviderAddTrustedMediator.csv}\dtRPATM
\pgfplotstableread[col sep=comma]{data/functions_general/setPenaltyRate.csv}\dtSPR
\pgfplotstableread[col sep=comma]{data/functions_general/setReactionDeadline.csv}\dtSRD

\catcode`\_=8 % category subscript

\begin{figure}
\begin{tikzpicture}
  \begin{axis}[
    boxplot/draw direction = y,
    xtick = {1,2,3,4,5,6,7},
    yticklabel style = {font=\footnotesize},
    xticklabel style = {align=center, font=\footnotesize, rotate=30},
    xticklabels = {JCaddTM, regJC, regM, regRP, RPaddTM, setPR, setRD},
    ylabel style = {font=\footnotesize},
    ylabel = {Duration [s]},
    ymax = 45, 
    cycle list = {set1-blue}, 
    height=.5\columnwidth,
    width=\columnwidth
    ]
    \addplot+[boxplot, fill, draw=black] table[ y = {dt}] {\dtJCATM};
    \addplot+[boxplot, fill, draw=black] table[ y = {dt}] {\dtRegJC};
    \addplot+[boxplot, fill, draw=black] table[ y = {dt}] {\dtRegM};
    \addplot+[boxplot, fill, draw=black] table[ y = {dt}] {\dtRegRP};
    \addplot+[boxplot, fill, draw=black] table[ y = {dt}] {\dtRPATM};
    \addplot+[boxplot, fill, draw=black] table[ y = {dt}] {\dtSPR};
    \addplot+[boxplot, fill, draw=black] table[ y = {dt}] {\dtSRD};
    
  \end{axis}
\end{tikzpicture}
\caption{Duration of \platform function calls during initial setup.}
\label{fig:dt-setup}
\end{figure}

==> implementation.tex <==
\section{\platform Implementation}
\label{sec:implementation}

In this section, we describe an implementation of \platform. It should be noted that other implementations of our architecture are also feasible. In this implementation, we use Ethereum as the distributed ledger and the core logic of the platform is implemented as an Ethereum smart contract (Section~\ref{sec:smartcontract}). %\Aron{I suggest omitting the following two sentences, this has already been established earlier.} \change{It provides interfaces for actors, to interact with the platform and thus each other. Additionally, it encodes the market rules, and checks the validity of offers.}{} 
%
\platform actors, including Job Creators, Resource Providers, Solvers and Directory services are implemented as Python services. These actors use the JSON-RPC interface to connect to the Ethereum Geth client \cite{geth}.  Note that each actor can be configured with any number of Geth clients and the ledger can be implemented as a private blockchain or we can use the main Ethereum chain as the ledger. All jobs in the current implementation are managed as Docker images since Docker provides a convenient way of measuring resource consumption, limiting it, and isolating the job from the host. 

%We also provide an  implementation of the entire \platform system, including all the actors and services. Note that there are other implementations of this architecture possible.


% In this section, we present this example implementation in detail.
% We implement \platform actors 
% as Python processes, which connect to Geth \cite{geth} to interact with the smart contract. 
% Our implementation is very flexible: each actor can be configured with any number of Geth clients and with a private blockchain or the main Ethereum chain.
%and listen for events on their configured Geth client. 



In this implementation, the storage of and access to data products for transmission between Resource Providers, Job Creators, and Mediators, are managed by the Directory service. Job Creators are permitted to publish data to Directories they choose to trust. When the Directory is notified that there is a new JC that trusts it, the Directory creates a new user account for that JC. The name of the user account is derived from the JC's Ethereum address.

%The Directory service also creates a unique SSH key and sends the private key back to the JC to use when uploading data products for jobs.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\columnwidth]{figures/directory.png}
    \caption{Directory contents for a Job Creator. The tar file is a Docker image, while \texttt{offer100} is a specific job offer. % The specific job offer is 100 and the matrix\_multiplication is the job tag. The tar file is the Docker image. 
    }
    \label{fig:directory}
\end{figure}

Job Creators (JC) are implemented as long-running processes, which can be managed using \emph{systemd} and provide a command line interface for submitting new job offers. Additionally, we provide a wrapper for Docker image creation and execution, which is used to prepare jobs for deployment. To determine job requirements jobs are profiled using the cli to execute them and monitor their resource utilization with cAdvisor \cite{cadvisor}. To submit a new job, a JC  creates a job identifier with the Directory where the files and Docker images can be uploaded (using the key received from Directory service). This job identifier can be later used with multiple job offers. The implementation supports changing the input files for different instances of the same job identifier. The input files are stored in a folder specific to the job offer. Figure~\ref{fig:directory} shows the contents of a folder for a JC a Directory service for one experiment.

Resource Providers (RP) also get a user account and SSH key from the Directory service. Once a job is matched, the Directory service receives the notification from the smart contract and grants read-only access to the files associated with that job to the RP. Results from the RP are similarly transferred to the matched JC. Mediators get access to corresponding job and result folders on the Directory when they are assigned to mediate a dispute. 

We provide a standalone Solver implementation, which tries to match offers as soon as they are posted. The present iteration uses a simple greedy matching algorithm to pair job and resource offers, but this is not a requirement. 

% \Aron{move to future work?} \ad{Sure}
% Other mechanisms could be implemented, such as solving periodically. \textcolor{blue}{} \Aron{We should discuss this in more detail as future work.}

%To provide this access, it uses \Aron{do we need implementation details like this?}Linux groups. T
%he Resource Provider also has a similar folder hierarchy in its account on the Directory, which can be used later to transfer result files. The directory service gives read only access to the result folder to the Job Creator


%specifies the \Aron{what is a tag?}tag of the job and uploads the files and Docker image of the job to the Directory service using SFTP (using the key received from Directory service). All new Job offers specify the job tag (a tag can be reused multiple times) and specify the input files. The input files are stored in a folder specific to the job offer. Figure~\ref{fig:directory} shows the contents of a folder for a Job Creator on the directory service for one experiment.}

%\Aron{Trusted by whom?! Trusted to do what?}


%is trusted it creates a new folder with SSH access permissions allowing the Job Creator to publish jobs. Permission is granted to a specific job folder for a Resource Provider when the Directory receives a notification that a match has been made, or for a Mediator when mediation is requested. 




%Job Creators consist of a Job Creator Daemon which is a long running process that has a CLI interface to submit new job offers. Additionally we provide a wrapper for Docker image creation and execution which is used to prepare jobs for deployment. There is also a script to execute and profile the jobs to determine their requirements which makes use of cAdvisor.  

%Resource Providers are implemented as Python processes. They consist of a wrapper that provides an interface to specify the chosen strategy. 

% Mediators are implemented as Python processes.
% \Aron{Let's just say that all actors are implemented as Python processes, instead of listing them one-by-one.}




% \textcolor{red}{To publish a job to a Directory the jobcreator actors specify the path to the job folder on the directory machine and the job tag. The input folder contain

% ocal path to the job, the job's tag, 
% the jobs specify a uniform Docker image via a tag.
% the input folder contains a json file that specifies the dimensions of two matrices. 
% The task is to do matrix multiplication of those two matrices. 
% The Directory has a creates a user for each wallet and a folder for each job submitted by that wallet. The folder contains the image as a .tar file and another folder for the job inputs. Before posting a new job off offer to the platform an actor can upload a new image, input folder, or both to the Directory.  
% }
% % There is also Docker wrapper for image creation and execution.\Aron{I don't think that we have space for minor implementation details.}

\subsection{Experiments with \platform}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/bbb.jpg}
    \caption{32 node BeagleBone cluster.}
    \label{fig:bbb}
%  \includegraphics[width=\columnwidth]{figures/cluster.pdf}
%     \caption{Topology of physical network connections.}
%     \label{fig:phy_topo}
\end{figure}

We chose to experiment and evaluate the overhead and operational performance of \platform on a 32 node BeagleBone ARM cluster (shown in Figure \ref{fig:bbb}) since many IoT  devices are ARM machines.  All nodes run Ubuntu 18.04. We ran a single instance of the Ethereum Geth client on the cluster master (an Intel machine running Linux). We used a script to control the operation of Resource Providers and Job Creators, assigned to different BeagleBone nodes as noted in the experiments below. The code and further experimental results are available on GitHub~\cite{modicum}. \taha{Change ``\textit{Mediation requested}`` to ``\textit{rejectResult}`` in Table~\ref{tab:Experiment3}}

In our initial experiments, we create a Job Creator and multiple Resource Providers, each running on a separate BeagleBone. The Job Creators and Resource Providers all have unique Ethereum accounts. The Mediator is run on a BeagleBone machines as well.  The Directory service runs on the cluster master. 
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth,trim={0.08cm 0.27cm 0.6cm 0.3cm},clip]{newResults/chart.pdf}
    \caption{Time series of platform events with one job offer and one resource offer  (Experiment 1). The horizontal axis shows the sequence of events, while the vertical axis shows the absolute wall clock time of events in 24-hour format.}
    \label{fig:J1R1l}
\end{figure*}

The job we chose for the evaluation is a Python program that performs matrix operations on matrices of different sizes. We set up the program so that the job size can be parameterized using an input JSON file, which is passed to the Resource Providers via the Directory. 

\begin{table}[t]
\caption{Mediation Sequence for Experiment 3. Mediation assignment took around 50 seconds.}
\label{tab:Experiment3}
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\footnotesize
\textbf{Time} & \textbf{Actor} & \textbf{Event}          & \textbf{Job id} \\ \hline
02:22:46      & JC             & Mediation requested     & 0               \\ \hline
02:22:46      & JC             & Mediation requested     & 1               \\ \hline
02:23:21      & JC             & Mediation requested     & 2               \\ \hline
02:23:21      & JC             & Mediation requested     & 3               \\ \hline
02:23:36      & JC             & JobAssignedForMediation & 0               \\ \hline
02:23:36      & JC             & JobAssignedForMediation & 1               \\ \hline
02:23:58      & JC             & JobAssignedForMediation & 2               \\ \hline
02:23:58      & JC             & JobAssignedForMediation & 3               \\ \hline
02:23:36      & Mediator       & Mediation Started       & 0               \\ \hline
02:23:38      & Mediator       & Mediation Started       & 1               \\ \hline
02:23:59      & Mediator       & Mediation Started       & 2               \\ \hline
02:23:59      & Mediator       & Mediation Started       & 3               \\ \hline
\end{tabular}

\end{table}

\textbf{Experiment 1:} Our first experiment involves a single Job Creator and a single Resource Provider. Both actors post one offer each, which are then matched to each other, resulting in the RP executing the job. Figure \ref{fig:J1R1l} shows the sequence of events from this experiment with wall-clock times.
%their sequence and the time between two events. 
The execution of the entire experiment from deploying the \platform smart contract to closing the match took less than 5 minutes, which includes mining on a private Ethereum network to record transactions on the ledger. %, took The full run of the system including mining of smart contract transactions finished within 5 minutes in this run.

\textbf{Experiment 2:}
% \textcolor{red}{
% jobs of different sizes
% how long to run job locally
% RPs already have base image, just need to get input
% JC has already published image. Not included because its just SFTP protocol overhead and only contributes to the first time an image is executed and can be accounted for in the offers. 2 mallicios 3 vary size }
In this experiment, we evaluate the duration and variability of key events on the platform. To this end, we created a script that generates a sequence of calls to the command line interface to publish matrix operation jobs to the Directory and post resource and job offers to \platform.
We repeat the experiment with jobs of different sizes and measure the time taken during various stages of the workflow (Figure \ref{fig:seqdiag}). When submitting jobs, we allow the Job Creator to pre-publish the Docker image to a Directory service that it trusts, and we also allow the Resource Providers to preload the Docker image. Results are shown in Figure~\ref{fig:exp2-1}. The matrix sizes were 100 square, 500 square, and 1000 square. The latter was the largest that we could process on a BeagleBone Black without memory mapping. Each of these runs consisted of 24 job offers and 24 resource offers, where 4 job offers were posted by a single Job Creator, and then 4 individual Resource Providers would post a single offer each, repeated 6 times. This sequence was the cause for some of the variability in the match time (c) and job completion time (f) since the first job offer must wait for at least 3 other job offers to be posted, while the fourth job offer has to wait only for a match. The second source of variability is the non-deterministic nature of mining a block, which results in variable transaction times.
%All the resource offers were identical as were the job offers, since we are interested in the variance. 

%This experiment had two phases, one in which we submitted several bad jobs by not publishing the docker container resulting in a JobNotFound error, and another where we submitted correct jobs. When submitting the correct jobs we allowed the Job Creator to have the docker image pre-published to the Directory service that it trusts, and we also allow the Resource Providers to have the docker image pre-loaded.

\textbf{Experiment 3:} In the third experiment, we set up four Resource Providers, which post one resource offer each, and one Job Creator, which posts four job offers. The Job Creator intentionally does not provide the job image files and asks for mediation when the Resource Providers report the error. Table~\ref{tab:Experiment3} shows the event sequence. The time between the mediation request and mediation execution varies slightly. This is primarily due to  waiting for the transaction (request to the smart contract) to be mined. In all four cases, the mediator correctly blames the Job Creator.




\begin{figure*}
    \centering
\begin{tikzpicture}
\begin{axis}[
      width=0.37\textwidth,
      height=0.23\textwidth,
      font=\footnotesize,
      grid=major,
      xtick={0,20,40,60,100,120,200,300},
      JobOfferStyle/.style={boxplot={box extend=0.5,}, blue, solid, fill=blue!20, mark=x},
      ytick={1, 2, 3, 4, 5, 6, 7},
      yticklabels={{(a)}, {(b)}, {(c)}, {(d)}, {(e)}, {(f)},{(g)}},
       ResourceOfferStyle/.style={boxplot={box extend=0.5,}, brown, solid, fill=brown!20, mark=x},
      RegisterStyle/.style={boxplot={box extend=0.5,}, black, solid, fill=blue!20, mark=x},
      MediatorStyle/.style={boxplot={box extend=0.5,}, green, solid, fill=green!20, mark=x},
      OfferMatchTimeStyle/.style={boxplot={box extend=0.5,}, red, solid, fill=red!20, mark=x},
      ResultTimeStyle/.style={boxplot={box extend=0.5,}, gray, solid, fill=gray!20, mark=x},
      ExecutionTimeStyle/.style={boxplot={box extend=0.5,}, orange, solid, fill=orange!20, mark=x},
      xlabel={matrices of size 100x100}
    %   xlabel={Job Offer Registration Time(\begin{tikzpicture}\draw [blue, fill=blue!20] (0pt,0pt) -- (5pt,0pt) -- (5pt,5pt) -- (0pt,5pt) -- (0pt,0pt);\end{tikzpicture}) and Offer Match Time (\begin{tikzpicture}\draw [red, fill=red!20] (0pt,0pt) -- (5pt,0pt) -- (5pt,5pt) -- (0pt,5pt) -- (0pt,0pt);\end{tikzpicture})},
    %   legend pos=north east,
    ]
    % \addplot+[JobOfferStyle, boxplot={draw position=1}] table [col sep=comma, y=JobOfferPostTime] {results/24J4R-1/JOO.csv};
    %  \addplot+[ResourceOfferStyle, boxplot={draw position=2}] table [col sep=comma, y=ResourceOfferPostTime] {results/24J4R-1/RPO.csv};
    %  \addplot+[OfferMatchTimeStyle, boxplot={draw position=3}] table [col sep=comma, y=OfferMatchTime] {results/24J4R-1/Match.csv};
    %  \addplot+[RegisterStyle, boxplot={draw position=4}] table [col sep=comma, y=RegistrationTime] {results/24J4R-1/Register.csv};
    %   \addplot+[MediatorStyle, boxplot={draw position=5}] table [col sep=comma, y=MediationTime] {results/24J4R-1/MediatorAddition.csv};
    %   \addplot+[ResultTimeStyle, boxplot={draw position=6}] table [col sep=comma, y=JobCompletionTime] {results/24J4R-1/Result.csv};
      
      \addplot+[JobOfferStyle, boxplot={draw position=1}] table [col sep=comma, y=JobOfferPostTime] {newResults/24J4R-100/JOO.csv};
     \addplot+[ResourceOfferStyle, boxplot={draw position=2}] table [col sep=comma, y=ResourceOfferPostTime] {newResults/24J4R-100/RPO.csv};
     \addplot+[OfferMatchTimeStyle, boxplot={draw position=3}] table [col sep=comma, y=OfferMatchTime] {newResults/24J4R-100/Match.csv};
     \addplot+[RegisterStyle, boxplot={draw position=4}] table [col sep=comma, y=RegistrationTime] {newResults/24J4R-100/Register.csv};
      \addplot+[MediatorStyle, boxplot={draw position=5}] table [col sep=comma, y=MediationTime] {newResults/24J4R-100/MediatorAddition.csv};
      \addplot+[ResultTimeStyle, boxplot={draw position=6}] table [col sep=comma, y=JobCompletionTime] {newResults/24J4R-100/Result.csv};
      \addplot+[ExecutionTimeStyle, boxplot={draw position=7}] table [col sep=comma, y=ExecutionTime] {newResults/24J4R-100/ExecutionTime.csv};
      
\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[
  width=0.37\textwidth,
      height=0.23\textwidth,
      font=\footnotesize,
      grid=major,
      JobOfferStyle/.style={boxplot={box extend=0.5,}, blue, solid, fill=blue!20, mark=x},
      ytick={1, 2, 3, 4, 5, 6, 7},
       xtick={0,20,40,60,100,120,200,300},
      yticklabels={{(a)}, {(b)}, {(c)}, {(d)}, {(e)}, {(f)},{(g)}},
       ResourceOfferStyle/.style={boxplot={box extend=0.5,}, brown, solid, fill=brown!20, mark=x},
      RegisterStyle/.style={boxplot={box extend=0.5,}, black, solid, fill=blue!20, mark=x},
      MediatorStyle/.style={boxplot={box extend=0.5,}, green, solid, fill=green!20, mark=x},
      OfferMatchTimeStyle/.style={boxplot={box extend=0.5,}, red, solid, fill=red!20, mark=x},
      ResultTimeStyle/.style={boxplot={box extend=0.5,}, gray, solid, fill=gray!20, mark=x},
      ExecutionTimeStyle/.style={boxplot={box extend=0.5,}, orange, solid, fill=orange!20, mark=x},
        xlabel={matrices of size 500x500}
    %   xlabel={Job Offer Registration Time(\begin{tikzpicture}\draw [blue, fill=blue!20] (0pt,0pt) -- (5pt,0pt) -- (5pt,5pt) -- (0pt,5pt) -- (0pt,0pt);\end{tikzpicture}) and Offer Match Time (\begin{tikzpicture}\draw [red, fill=red!20] (0pt,0pt) -- (5pt,0pt) -- (5pt,5pt) -- (0pt,5pt) -- (0pt,0pt);\end{tikzpicture})},
    %   legend pos=north east,
    ]
    % \addplot+[JobOfferStyle, boxplot={draw position=1.15}] table [col sep=comma, y=JobOfferPostTime] {results/24J4R-500/JOO.csv};
    %  \addplot+[ResourceOfferStyle, boxplot={draw position=1.85}] table [col sep=comma, y=ResourceOfferPostTime] {results/24J4R-500/RPO.csv};
    %  \addplot+[OfferMatchTimeStyle, boxplot={draw position=3.15}] table [col sep=comma, y=OfferMatchTime] {results/24J4R-500/Match.csv};
    %  \addplot+[RegisterStyle, boxplot={draw position=3.85}] table [col sep=comma, y=RegistrationTime] {results/24J4R-500/Register.csv};
    %   \addplot+[MediatorStyle, boxplot={draw position=5.15}] table [col sep=comma, y=MediationTime] {results/24J4R-500/MediatorAddition.csv};
    %   \addplot+[ResultTimeStyle, boxplot={draw position=5.85}] table [col sep=comma, y=JobCompletionTime] {results/24J4R-500/Result.csv};
      
    \addplot+[JobOfferStyle, boxplot={draw position=1}] table [col sep=comma, y=JobOfferPostTime] {newResults/24J4R-500/JOO.csv};
     \addplot+[ResourceOfferStyle, boxplot={draw position=2}] table [col sep=comma, y=ResourceOfferPostTime] {newResults/24J4R-500/RPO.csv};
     \addplot+[OfferMatchTimeStyle, boxplot={draw position=3}] table [col sep=comma, y=OfferMatchTime] {newResults/24J4R-500/Match.csv};
     \addplot+[RegisterStyle, boxplot={draw position=4}] table [col sep=comma, y=RegistrationTime] {newResults/24J4R-500/Register.csv};
      \addplot+[MediatorStyle, boxplot={draw position=5}] table [col sep=comma, y=MediationTime] {newResults/24J4R-500/MediatorAddition.csv};
      \addplot+[ResultTimeStyle, boxplot={draw position=6}] table [col sep=comma, y=JobCompletionTime] {newResults/24J4R-500/Result.csv};
      \addplot+[ExecutionTimeStyle, boxplot={draw position=7}] table [col sep=comma, y=ExecutionTime] {newResults/24J4R-500/ExecutionTime.csv};
      

\end{axis}
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[
  width=0.37\textwidth,
      height=0.23\textwidth,
      font=\footnotesize,
      grid=major,
       xtick={0,20,40,60,100,150,200,250,300},
      JobOfferStyle/.style={boxplot={box extend=0.5,}, blue, solid, fill=blue!20, mark=x},
      ytick={1, 2, 3, 4, 5, 6, 7},
      yticklabels={{(a)}, {(b)}, {(c)}, {(d)}, {(e)}, {(f)},{(g)}},
       ResourceOfferStyle/.style={boxplot={box extend=0.5,}, brown, solid, fill=brown!20, mark=x},
      RegisterStyle/.style={boxplot={box extend=0.5,}, black, solid, fill=blue!20, mark=x},
      MediatorStyle/.style={boxplot={box extend=0.5,}, green, solid, fill=green!20, mark=x},
      OfferMatchTimeStyle/.style={boxplot={box extend=0.5,}, red, solid, fill=red!20, mark=x},
      ResultTimeStyle/.style={boxplot={box extend=0.5,}, gray, solid, fill=gray!20, mark=x},
      ExecutionTimeStyle/.style={boxplot={box extend=0.5,}, orange, solid, fill=orange!20, mark=x},
        xlabel={matrices of size 1000x1000}
    %   xlabel={Job Offer Registration Time(\begin{tikzpicture}\draw [blue, fill=blue!20] (0pt,0pt) -- (5pt,0pt) -- (5pt,5pt) -- (0pt,5pt) -- (0pt,0pt);\end{tikzpicture}) and Offer Match Time (\begin{tikzpicture}\draw [red, fill=red!20] (0pt,0pt) -- (5pt,0pt) -- (5pt,5pt) -- (0pt,5pt) -- (0pt,0pt);\end{tikzpicture})},
    %   legend pos=north east,
    ]
    % \addplot+[JobOfferStyle, boxplot={draw position=1.15}] table [col sep=comma, y=JobOfferPostTime] {results/24J4R-1000/JOO.csv};
    %  \addplot+[ResourceOfferStyle, boxplot={draw position=1.85}] table [col sep=comma, y=ResourceOfferPostTime] {results/24J4R-1000/RPO.csv};
    %  \addplot+[OfferMatchTimeStyle, boxplot={draw position=3.15}] table [col sep=comma, y=OfferMatchTime] {results/24J4R-1000/Match.csv};
    %  \addplot+[RegisterStyle, boxplot={draw position=3.85}] table [col sep=comma, y=RegistrationTime] {results/24J4R-1000/Register.csv};
    %   \addplot+[MediatorStyle, boxplot={draw position=5.15}] table [col sep=comma, y=MediationTime] {results/24J4R-1000/MediatorAddition.csv};
    %   \addplot+[ResultTimeStyle, boxplot={draw position=5.85}] table [col sep=comma, y=JobCompletionTime] {results/24J4R-1000/Result.csv};
      
      
      \addplot+[JobOfferStyle, boxplot={draw position=1}] table [col sep=comma, y=JobOfferPostTime] {newResults/24J4R-1000/JOO.csv};
     \addplot+[ResourceOfferStyle, boxplot={draw position=2}] table [col sep=comma, y=ResourceOfferPostTime] {newResults/24J4R-1000/RPO.csv};
     \addplot+[OfferMatchTimeStyle, boxplot={draw position=3}] table [col sep=comma, y=OfferMatchTime] {newResults/24J4R-1000/Match.csv};
     \addplot+[RegisterStyle, boxplot={draw position=4}] table [col sep=comma, y=RegistrationTime] {newResults/24J4R-1000/Register.csv};
      \addplot+[MediatorStyle, boxplot={draw position=5}] table [col sep=comma, y=MediationTime] {newResults/24J4R-1000/MediatorAddition.csv};
      \addplot+[ResultTimeStyle, boxplot={draw position=6}] table [col sep=comma, y=JobCompletionTime] {newResults/24J4R-1000/Result.csv};
      \addplot+[ExecutionTimeStyle, boxplot={draw position=7}] table [col sep=comma, y=ExecutionTime] {newResults/24J4R-1000/ExecutionTime.csv};
      

\end{axis}
\end{tikzpicture}
\caption{Results from Experiment 2.   The horizontal axis is the elapsed time in seconds. The values shown from bottom to top are: (a) time to register job offer, (b) time to register resource offer, (c) time to match offers (measured from when offers were issued), (d) time to register all actors, (e) time to select mediators before posting job offer, (f) time to complete job (measured from when the job was first posted), and (g) the execution time of the job.}
\label{fig:exp2-1}
\end{figure*}

%\subsection{Experimental Setup}
%\Aron{Let's separate implementation and experimental setup.} 





% \begin{figure}
%     \centering
% \begin{tikzpicture}
% \begin{axis}[
%   width=0.48\textwidth,
%       height=0.3\textwidth,
%       font=\footnotesize,
%       grid=major,
%       JobOfferStyle/.style={boxplot={box extend=0.5,}, blue, solid, fill=blue!20, mark=x},
%       ytick={1, 2, 3, 4, 5, 6},
%       yticklabels={{(a)}, {(b)}, {(c)}, {(d)}, {(e)}, {(f)}},
%       ResourceOfferStyle/.style={boxplot={box extend=0.5,}, brown, solid, fill=brown!20, mark=x},
%       RegisterStyle/.style={boxplot={box extend=0.5,}, black, solid, fill=blue!20, mark=x},
%       MediatorStyle/.style={boxplot={box extend=0.5,}, green, solid, fill=green!20, mark=x},
%       OfferMatchTimeStyle/.style={boxplot={box extend=0.5,}, red, solid, fill=red!20, mark=x},
%       ResultTimeStyle/.style={boxplot={box extend=0.5,}, gray, solid, fill=gray!20, mark=x},
%     %   xlabel={Job Offer Registration Time(\begin{tikzpicture}\draw [blue, fill=blue!20] (0pt,0pt) -- (5pt,0pt) -- (5pt,5pt) -- (0pt,5pt) -- (0pt,0pt);\end{tikzpicture}) and Offer Match Time (\begin{tikzpicture}\draw [red, fill=red!20] (0pt,0pt) -- (5pt,0pt) -- (5pt,5pt) -- (0pt,5pt) -- (0pt,0pt);\end{tikzpicture})},
%     %   legend pos=north east,
%     ]
%     \addplot+[JobOfferStyle, boxplot={draw position=1.15}] table [col sep=comma, y=JobOfferPostTime] {results/24J4R-500/JOO.csv};
%      \addplot+[ResourceOfferStyle, boxplot={draw position=1.85}] table [col sep=comma, y=ResourceOfferPostTime] {results/24J4R-500/RPO.csv};
%      \addplot+[OfferMatchTimeStyle, boxplot={draw position=3.15}] table [col sep=comma, y=OfferMatchTime] {results/24J4R-500/Match.csv};
%      \addplot+[RegisterStyle, boxplot={draw position=3.85}] table [col sep=comma, y=RegistrationTime] {results/24J4R-500/Register.csv};
%       \addplot+[MediatorStyle, boxplot={draw position=5.15}] table [col sep=comma, y=MediationTime] {results/24J4R-500/MediatorAddition.csv};
%       \addplot+[ResultTimeStyle, boxplot={draw position=5.85}] table [col sep=comma, y=JobCompletionTime] {results/24J4R-500/Result.csv};
      

% \end{axis}
% \end{tikzpicture}
% \caption{24 Jobs, 4 resource providers with matrices of size 500x500}
% \end{figure}


% \begin{figure}
%     \centering
% \begin{tikzpicture}
% \begin{axis}[
%   width=0.48\textwidth,
%       height=0.3\textwidth,
%       font=\footnotesize,
%       grid=major,
%       JobOfferStyle/.style={boxplot={box extend=0.5,}, blue, solid, fill=blue!20, mark=x},
%       ytick={1, 2, 3, 4, 5, 6},
%       yticklabels={{(a)}, {(b)}, {(c)}, {(d)}, {(e)}, {(f)}},
%       ResourceOfferStyle/.style={boxplot={box extend=0.5,}, brown, solid, fill=brown!20, mark=x},
%       RegisterStyle/.style={boxplot={box extend=0.5,}, black, solid, fill=blue!20, mark=x},
%       MediatorStyle/.style={boxplot={box extend=0.5,}, green, solid, fill=green!20, mark=x},
%       OfferMatchTimeStyle/.style={boxplot={box extend=0.5,}, red, solid, fill=red!20, mark=x},
%       ResultTimeStyle/.style={boxplot={box extend=0.5,}, gray, solid, fill=gray!20, mark=x},
%     %   xlabel={Job Offer Registration Time(\begin{tikzpicture}\draw [blue, fill=blue!20] (0pt,0pt) -- (5pt,0pt) -- (5pt,5pt) -- (0pt,5pt) -- (0pt,0pt);\end{tikzpicture}) and Offer Match Time (\begin{tikzpicture}\draw [red, fill=red!20] (0pt,0pt) -- (5pt,0pt) -- (5pt,5pt) -- (0pt,5pt) -- (0pt,0pt);\end{tikzpicture})},
%     %   legend pos=north east,
%     ]
%     \addplot+[JobOfferStyle, boxplot={draw position=1.15}] table [col sep=comma, y=JobOfferPostTime] {results/24J4R-1000/JOO.csv};
%      \addplot+[ResourceOfferStyle, boxplot={draw position=1.85}] table [col sep=comma, y=ResourceOfferPostTime] {results/24J4R-1000/RPO.csv};
%      \addplot+[OfferMatchTimeStyle, boxplot={draw position=3.15}] table [col sep=comma, y=OfferMatchTime] {results/24J4R-1000/Match.csv};
%      \addplot+[RegisterStyle, boxplot={draw position=3.85}] table [col sep=comma, y=RegistrationTime] {results/24J4R-1000/Register.csv};
%       \addplot+[MediatorStyle, boxplot={draw position=5.15}] table [col sep=comma, y=MediationTime] {results/24J4R-1000/MediatorAddition.csv};
%       \addplot+[ResultTimeStyle, boxplot={draw position=5.85}] table [col sep=comma, y=JobCompletionTime] {results/24J4R-1000/Result.csv};
% \end{axis}
% \end{tikzpicture}
% \caption{24 Jobs, 4 resource providers with matrices of size 1000x1000}
% \end{figure}

% In al


% For the simulation we use a simple script that calls the CLI to submit jobs specified in a job schedule.
% RPs : In this simulation we use a prescriptive time series strategy specify how many resources are available and when. To monitor resource consumption we use cAdvisor. 

\iffalse
\subsection{Results}
\label{sec:experimental}


\subsection{Performance}
average job execution time with error bars for a specific job (native Docker, Ethereum, Modicum)

average job execution time vs job size(native Docker, Ethereum, Modicum)

resource utilization (bandwidth, storage, network?) (native Docker, Ethereum, Modicum)

\subsection{Market Health}
\#jobs completed/\#jobs input as the simulation progresses

\# faulty nodes (tunable parameter)

money flow as the simulation progresses

% \section{Discussion/Comparison}
% \label{sec:compare}

% \begin{table}[t]
% \centering
% \begin{tabulary}{\textwidth}{|c|L|l|}%lower case means no linebreak, upper case allows line breaks
% \hline
% \multicolumn{3}{|c|}{Quantitative Comparison} \\
% \hline
%  &  \# or replications& \\
% \hline
% Ethereum & & \\
% Hyperledger & & \\ 
% TrueBit & & \\ 
% \hline
% \end{tabulary}
% \end{table}

\fi

==> intro_old.tex <==
\section{Introduction}
\label{sec:intro}
{\bf Emerging Trends} The emerging trend in the distributed computing paradigm with the recent progress in Internet of Things and widespread sensor integration is the concept of bringing computing to the edge of the physical systems -- wherein the edge implies closer to the source of the physical phenomena. Consequently a number of cities and vendors are increasingly deploying smart devices over large widespread urban and rural geographical areas in anticipation of increasing workload. The manifestation of these trends have been given different names in the community: Fog computing, cloudlets, micro data centers etc \cite{garcia-valls_introducing_2018}. 

However, there are still fundamental challenges which are not being addressed. For example, while the computing resources are becoming highly available, they are heterogeneous and distributed over large areas across different networks and probably owned by different organizations. Prior work on resource allocation of tasks has focused primarily on specific isolated problem instances, such as knapsack [Moser et al. 1997, Mostofa et al. 2006] or Constraint Satisfaction Problem (CSP) approaches [Van Hentenryck 1989] for solving network/sensor resource allocation [Navaie and Yanikomeroglu, 2006, Shabany et al. 2004, Song et al. 2008, Pradhan et.al 2016] or bin-packing algorithms for multiprocessor scheduling [Aydin et al. 2001, Boland 2001, Chekuri et al. 2004, Coffman et al. 1978, Gillespie 2001, Ritchie 2003, Roy et.al 2011, Turner and White 2013]. 

Large-scale  resource allocation decisions for systems, which require coordinated solving of multiple large-scale resource allocation sub-problems have not been thoroughly considered, particularly when incomplete or incorrect system knowledge may be present. Isolated instances of linked resource allocation problems, such as the linked knapsack resource allocation problems and linked queuing theoretic formulations [Dubey et.al 2009,2010, Gandhi et.al 2012] have shown good results but not been employed at the level of dynamism and complexity seen in large edge computing deployments. CSP solvers used in general solution approaches, such as branch and bound optimization [Lawler and Wood 1966, Narendra and Fukunaga 1977], are typically used for general constraint satisfaction problems that do not fit within the classical mold of bin-packing, satisfiability, knapsack, or other classical problem definitions. A fundamental issue with these approaches is that they typically do not scale well for complex resource allocation problems, particularly at the problem sizes needed to manage city or country-scale resource allocation decisions.

Our vision is to formulate a decentralized management framework that allows for resource allocation of tasks as a market problem, leaving the discovery of resources and management of tasks directly to the computing nodes.  This approach is more realistic than models based on simplified assumptions about resource reliability and allocation, such as bin-packing, knapsacks, constraint satisfaction problems, or other meta heuristic models. The market based approach is appealing because they provide some key properties, including the behavior of collapsing to a Nash equilibrium, which can be designed, assuming rational participants. It also provides a consistent interface to interact with diverse organizations, as well as provide incentives for participation. The market then becomes the entity that defines constraints, objective functions, and other key decisions that allow us to reason about: (1) what resources are available in the environment; (2) how likely each resource is to change in a significant manner in the next time epoch; (3) how fast resources can be allocated and released; (4) critical task failure; and (5) how damaging having insufficient resources would be to an individual entity or to the system itself where damage is quantified by an economic metric. 

While market based approaches are advantageous in dispersing the management responsibility to individual agents the still suffer from the possibility of malicious behavior. Consider the case where a resource provider might knowingly or unknowingly provide wrong computation results or try to game the market by bidding on tasks but never completing them. Classically in distributed computing systems such problems have been solved using consensus algorithms. Two algorithms of specific interest to us are Practical Byzantine Fault Tolerance (PBFT) [liskov] and Proof of Work [blockchain]. The most popular distributed computing frameworks built on these consensus algorithms are frabric (hyperledger) and Ethereum. They provide a trust-less distributed computer along with  financial incentives to participate. On the other side of the spectrum are volunteer computing solutions such as BOINC that do not provide any consensus guarantees and are therefore not of interest to us. Further, these architectures do not include incentives, removing the primary motivation to behave selfishly, however this strength is also a weakness in that there is limited participation and in turn limited computational power available. Hence we only focus on consensus driven distributed computing solutions.

The current problem with Etheruem [need to say something about frabric] is that it suffers from the the same issues as Bitcoin, namely excessive power consumption due to inefficient computation. The reason for the inefficiency is derived from the fundamental assumption that there are no trusted nodes, which means that to achieve global consensus all participants must duplicate every instruction. \textcolor{red}{expand on BFT consensus}. There have been some efforts to ameliorate the situation, for example TrueBit, which performs computations using a typical computer and only relies on the distributed computer to complete disputed instructions, however this approach is still quite inefficient. They address this through incentives and security deposits but the economic analysis provided is not convincing as we will show in section \ref{sec:related}. We will also evaluate the degree of the computational inefficiency of their approach in our related work. There are other market-based solutions \textcolor{red}{such as...} which we will also discuss in section \ref{sec:related}, along with their respective disadvantages.




%Thus, trying to manage them centrally like a cloud computing resource is not feasible. Essentially, this requires decentralized management for which market based approach is an alternative. Markets are appealing because they provide some key properties, including the behavior of collapsing to a Nash equilibrium, which can be designed, assuming rational participants. It also provides a consistent interface to interact with diverse organizations, as well as incentives for participation.

%The most popular distributed computer currently is Ethereum. It is popular because it is the first successful implementation of a trust-less distributed computer and it provides strong financial incentives to participate. However it suffers from the the same issues as Bitcoin, namely excessive power consumption due to inefficient computation. The reason for the inefficiency is derived from the fundamental assumption that there are no trusted nodes, which means that to achieve global consensus all participants must duplicate every instruction. \textcolor{red}{expand on BFT consensus}

%https://hgf18.sched.com/event/JKT1/beyond-consensus-in-permissioned-ledgers-alysson-bessani-university-of-lisbon -- this guys works on PBFT derived consensus for hyperledger.



% In addition to market based approaches, distributed solutions such as Volunteering Computing have also been explored in the past. Examples of this architecture include  BOINC \cite{boinc} \textcolor{red}{...other volunteer computing architectures}. 

{\bf Modicum Approach:} Our approach to decentralized outsourced computing at edge, in contrast to other market based approaches, emphasizes retaining the computational efficiency through the use of provisionally trusted mediators. Other current mechanisms require extensive duplication of computations, instead we use a mediator that duplicates the computation under contention and provides a ruling, allowing us to achieve consensus with only the single re-execution. %this can be relaxed somewhat if we want to do some PBFT among arbitrators if we are unwilling to trust them. 

% \textcolor{red}{TODO: take a look at that paper from ICPADS that talked about modifying PBFT with the addition of witnesses}

{\bf Our Contributions}

In this paper we 
\begin{enumerate*}
    \item present a market based architecture for distributed computing which differs from prior works  in that it maintains computational efficiency by utilizing a conditionally trusted mediator to achieve consensus, 
    \item provide a comprehensive economic analysis of our protocol, and an evaluation of the analysis presented in comparable works, and 
    \item we provide an implementation and an experimental evaluation of the proposed architecture.
\end{enumerate*}
  



% ParaDrop
% cloudlet
% BOINC
% sawtooth
% fogcoin
% SONM, Golem, iExec, TrueBit


% In recent years there has been a proliferation of "smart devices" that send data to remote centralized cloud servers for processing and synchronization between devices among other services. It has been estimated that the number of these devices will reach 30.7 billion by 2020\footnote{https://cdn.ihs.com/www/pdf/enabling-IOT.pdf}. This connectivity extends to smart cars, which are anticipated to generate 1.4 GB of data per second according to Intels's CEO\footnote{https://www.networkworld.com/article/3147892/internet/one-autonomous-car-will-use-4000-gb-of-dataday.html}, as well as cities such as Singapore, Dubai, and New York where smart city technologies have been implemented\footnote{https://en.wikipedia.org/wiki/Smart\_city}.

% Fog computing relies on distributed compute devices which may be owned  by a single organization [paradrop, municipality ] or not [volunteer  computing, some opportunistic cell phone user paper]. Since the compute resources are geographically distributed there are several challenges that make centralized management impractical. These challenges include 1) unreliable network connections, which impacts data transfer and may result in network partitions, 2) the nodes are dynamic and may enter and exit the system unpredictably, and 3) nodes may be malicious, either because They have become compromised, or are owned by a malicious user. All these challenges potentially lead to failure in the system, and  since we consider malicious nodes we must address byzantine failure.  These can be condensed into two main problems, 1) how can results from a  computation be trusted? and 2) how can we keep track of the  resources available in the system to allow the scheduling of jobs?  

% Result checking is generally addressed through replication of computation and consensus or  verification when possible. There are several algorithms that have  been developed to achieve consensus under byzantine failure including  RAFT, PBFT, Proof of Work, Proof of stake, and Delegated Proof of Stake mechanisms. Each of these algorithms make trade offs between efficiency of computation and reliability or trust worthiness of the results. In this work we present a system that achieves consistency through arbitration. \textcolor{red}{TODO: Compare big O of various protocols}

% In a centrally managed system the resources are known a priori, and discovery mechanisms may be used to provide health monitoring of the devices. In the environment we have described this approach can not work, One method to track resource availability  is to invert the problem by establishing a market where resource providers  post offers to use their resources and job creators post offers specifying the  jobs to run, pushing the responsibility of management back to the nodes.  Given a set of offers, traditional scheduling algorithms may be applied.

% In order to ascertain the feasibility of the architecture described a financial analysis is required to demonstrate that it is in the best interests of the participants to be honest. This will be shown later in the paper. 

\textcolor{red}{TODO: Outline}

==> proof.tex <==
% \documentclass[]{article}

% \usepackage{fullpage}
% \usepackage{amsmath}
% \usepackage{amsthm}
% \newtheorem{theorem}{Theorem}

% \newcommand{\Util}[1]{\ensuremath{\mathcal{U}_{#1}}}

% \title{\Large MODiCuM: Mechanisms for Outsourcing via a\\ Decentralized Computation Market\\[1em] \large Theorem 1}
% \date{}
% \author{Scott Eisele, Taha Eghtesad, Nicholas Troutman,\\Aron Laszka, Abhishek Dubey}

% \begin{document}

% \maketitle

Our goal is to characterize when neither actors have an incentive to act dishonest.
We capture this using the concept of Nash equilibrium.
Formally, strategy profile $(Cj, Cr)$ is a Nash equilibrium if neither actor can increase its own expected utility by unilaterally changing its strategy choice.

\begin{theorem}
\label{thm:NE}
Both RP and JC acting honestly is a Nash equilibrium if and only if
\begin{equation*}
   p  
    \leq 
    Q \frac{P_m \cdot (2 f + M + r) - r -f  }{ C_j}
\end{equation*}
and
\begin{equation*}
 p \geq \frac{(1 - Q)}{P_j} + \frac{C - C_d}{P_j \cdot (r + f + M)} .
\end{equation*}
\end{theorem}

\begin{proof}
First, JC will act honestly if and only if
\begin{align*}
    \Util{JC}(C_j, C_r) &\geq \Util{JC}(D_j, C_r) \\
    Q \cdot (B - r) + (1 - Q) \cdot f - p \cdot  C_j 
    &\geq 
    Q \cdot \big[ B + (1 - P_m) \cdot f  - P_m \cdot (f + M + r) \big] + (1 - Q) \cdot f .
    \end{align*}
Equivalently,
    \begin{align*}
    - p \cdot  C_j 
    &\geq 
    Q \cdot \big[ r + (1 - P_m) \cdot f  - P_m \cdot (f + M + r) \big] \\
     p  
    &\leq 
    Q \frac{P_m \cdot (f + M + r) - r - (1 - P_m) \cdot f}{ C_j} \\
     p  
    &\leq 
    Q \frac{P_m \cdot (2 f + M + r) - r -f  }{ C_j} .
\end{align*}

Second, the RP will act honestly if and only if
\begin{align*}
    \Util{RP}(C_j, C_r) &\geq \Util{RP}(C_j, D_r) \\
    Q \cdot r - (1 - Q) \cdot (f + M) - C 
    &\geq (1 - p \cdot P_j) \cdot r - p \cdot P_j \cdot (f + M) - C_d .
\end{align*}
Equivalently,
\begin{align*}
 p \cdot P_j \cdot (r +  f + M)
    &\geq (1 - Q) \cdot (f + M + r) + C - C_d \\ 
 p &\geq \frac{(1 - Q) \cdot (f + M + r) + C - C_d}{P_j \cdot (r + f + M)}  \\
 p &\geq \frac{(1 - Q)}{P_j} + \frac{C - C_d}{P_j \cdot (r + f + M)}.
\end{align*}
\end{proof}

\thispagestyle{empty}

% \end{document}


==> related.tex <==
\section{Related Work}
\label{sec:related}

%\subsubsection{Security}

Shan et al. gives a detailed survey of current security concerns and strategies for outsourcing potentially valuable data. The paper systematically explains a wide variety of known security vulnerabilities and provides applicable solutions \cite{shan2018practical}.

\subsection{Verification}

More applicable work has been recorded on the individual parts to make up this project, especially verification and data feed systems. Our implementation doesn't foresee the need for a data-feed system since offer posting, matching, and verification are all self contained. But plenty of data feed systems utilize a verification system that we can cannibalize and apply to out computational results.

Of the existing verification systems, our biggest influence was the TrueBit system, where the reward for verifying protested solutions was inversely proportional to the total number of active verifiers. This model ensures that the verification system will reach a desired equilibrium proportional to the reward structure.

There are a few plurality based verification systems that are simple to implement at the cost of redundant computation. Schelling Coin offers a novel verification system called the Schelling process. Multiple participants submit redundant values for a specific data feed. After submitting, each participant reports what value they believe is the median. Participants who submit a report within the allowable range of the true median will be rewarded. This process is vulnerable to a large-scale Sybil attacks, but offers an interesting crowd-sourced verification process \cite{lesaege2017short}.

%\Aron{``quote''}
Sabotage-Tolerance Mechanisms offers another democratic verification system. All submitters have a reputation score that affects the importance of their solutions. Each submitted answer is tabulated from it's distance to the ``correct'' solution and the submitter's reputation score is changed proportional to this distance. Reputations that fall below a break point cause the user to be banned from the system \cite{sarmenta2001sabotage}.

An alternative to plurality submissions, is Enclave hardware guarantors embedded in the hardware. Town Crier uses hardware guarantors as a verification system to reduce redundancy. Enclaves are not prevalent enough to require them now, though we may incorporate the addition of them in the future \cite{zhang2016town}.

By reducing the range of computational job properties, the jobs can be verified mathematically without re-computation \cite{ben2013snarks}. Computation program results can be transformed into a transcript of variable states at different checkpoints. Instead of reconciling the entire job, the transcript for the completed job can be queried and checked for completeness \cite{walfish2015verifying}.


\subsection{Economic Analysis}

Multiple papers have modeled economic systems and assigned optimal rewards and fine values. The most applicable has been  \cite{dong2017betrayal}, which sets up a Nash Equilibrium point to disincentive collusion and other hostile strategies. The paper gives a working model to plug in unique system constraints and variables, and has the advantage of only changing the payout and buy in value to control behavior. 

Optimal Contracts for Outsourced Computation describes multiple models of reward and fines in terms of multiple agents and strategies. Our economic model took cues from their models and incorporated a version of their single agent model and tweaked it to create our own analysis \cite{pham2014optimal}.

We ultimately decided on a market-based non-reputation system, but in the future we may implement reputation. In  \cite{belenkiy2008incentivizing}, agents are given a reputation score based on their earlier solutions. During plurality processes the reputation scores act as weights in achieving the final solution. Once a reputation score drops below a certain threshold the account is banned.

\subsection{Alternative Computational Marketplaces}

There have been multiple white papers and publications on a decentralized computational marketplace: namely iExec, SONM, and the Golem project \cite{brundo2018blockchain}.  Golem focuses in rendering and has taken a top-down approach to creating their platform, with the ultimate goal of creating a decentralized supercomputer \cite{Golem}. iExec takes a bottom-up philosophy, all transactions are through decentralized applications (Dapps), that anyone can create. iExec plans to be a blockchain-based distributed cloud with advanced Dapp functionality that caters to a large variety of projects \cite{iExec}. SONM (Supercomputer Organized by Network Mining) is a cryptocoin computation fog marketplace that has made it to market and uses the same Docker setup as our platform, but has several comparative disadvantages. There is no mention of verification systems for improper job computation in the SONM documentation. There is no obvious pipeline to flag a fraudulent account, and the only steps that are possible in the architecture is to freeze the accused party's wallet \cite{SONM}. \platform differentiates itself by focusing on an economically feasible and heavily verified marketplace for independent jobs. iExec's Dappstore and ubiquity allows the platform to compute a variety of processes without specializing in a peer-to-peer marketplace, Golem's more centralized supercomputer approach allows for larger more complicated processes specifically rendering, and while SONM is the closest to \platform, it lacks a rigorous verification system to enforce a healthy marketplace.

\subsection{Other}
Fogcoin\cite{fogcoin} is a crypto-currency that considers geographical distance properties between matches to minimize the cost of transmitting data. This principal can be extrapolated and applied to any transactional product \cite{brundo2018blockchain}.



==> reviews.tex <==

----------------------- REVIEW 1 ---------------------

Overall evaluation: -2 (reject)

----------- Overall evaluation -----------

Modicum is a system for supporting open and decentralized computing market for outsourcing. The mechanism is clearly defined. It also seems that a viable implementation is provided. However, I do have the following concerns.

(1) It seems that the problem and the mechanism is quite straightforward. 
Is this suitable as a research problem? \ise{contributions. Check, hightlight challenges if there is space}
What is the fundamental problem of building an outsourcing platform? \ise{intro. Check} \ise{@Abhishek, what do you think the fundamental problem of building an outsourcing platform is?}
% The current platform of Ethereum is quite slow. Will this influence the availability of Modicum? 
% \ise{not tied to ethereum(mentioned in future work,check for other mentions).}
% \ise{ethereum is improving(add to conclusion).}


% \ise{platform limitations got lost. They were before contribution in icdcs 2019.}
% \ise{job limitations: batch, not time critical, only supports deterministic jobs, does not provide confidentiality, In the current implementation, task confidentiality cannot be guaranteed since computation may be outsourced to any capable participant.}\ise{covered in III.A}
% \ise{does not prevent cheating and misuse only deters rational agents (add to intro)}

% Why not just use several centralized platforms for supporting outsourcing? The discussion in the paper does not provide enough insights.

% (1a) Our paper needs to discuss the design challenges in more detail. We had to put a lot of work into the design because we encountered a series of challenges, but only the "clean" end result was visible to the reviewer.
% We also need to discuss the advantages of a single large market compared to a number of smaller ones (economy of scale, non-fractured ecosystem, etc.).

% (2) Not quite sure about some of the assumptions in the paper. For example, while discussion about how to use the game theory for reason about the behavior, the Mediators are assumed to act correctly. And then, the Nash equilibrium is gotten in the case that JC and SP all act properly. However, if they both act properly, how Mediators can benefit? Mediators can get profit for nothing? \ise{in IV.c check that mediator's availability price is clear. Add nomenclature. Will analyze in future.}

% (2a) Good point. We actually discussed this (the solution is to simply add a fee for the availability of the reviewers), but if I remember correctly, we did not have to add it to the paper. Easy to fix.

% (3) If the system uses the Ethereum, the cost will be very high. Will the system still be beneficial? Will JC or SP pay the fee on Ethereum?

% (3a) Firstly, we can include transaction fees in the game theoretic analysis. 
% Second, we can also do a general feasibility analysis, where we consider the transaction costs associated with the entire workflow. \ise{covered in analysis. @Aron: check?}
% Third, we can include some real-world data, which at this point in time will not look good, as well as an overview of planned Ethereum developments, which are expected cut cost down significantly.\ise{covered in V.A. add citation to planned Ethereum developments.}

%(4) It seems that they way Modicum uses cryptography is problematic. In page 8, first paragraph says “The Directory service also creates a unique SSH key and sends the private key back to the JC to use when uploading data products for jobs.” Private keys should not be used in this way.
(5) The experiments are not convincing. It is hard to do evaluation while investigating about so large a system. However, the experiments now fail to provide enough information about the essential part outsourcing market. It is not clear that whether the simple example computing task can represent the typical workload for outsourcing or not. Is there any benchmark workload or typical workload in the literature that can be used to make a typical workload for evaluation? \ise{covered by V.A. We don't do large scale experiments because it would only test the smart contract capacity (and so ethereum) or the solver which is just $n^2$ complexity which is not going to be a bottle neck. Add if there is space.}

% (5a) We should definitely improve the experimental setup (again, this is something that we would have done if we had more time). We can use the traffic routing example that we have been planning for MODiCuM2 in the next submission (if our next submission includes services). A standard benchmark problem would be nice too. \ise{covered by comment above}

% (6) Since Modicum uses docker for hosting computing tasks, what is the typical size of the docker images? Will the size for downloading prevent the adopting the solution in the paper?\ise{covered in III.A,B and V.0}
% \ise{in III.A, resources}
% \ise{in III.B , prices, RP resources greater than JC requirements (mem, cpu, layers)}
% \ise{RP resources greater than JC requirements III.B.3}
% (6a) Again, this is something that we discussed. Our solution is to specify multiple Docker layers, some of which may be reused. We should include the solution in the next submission.

% ----------------------- REVIEW 2 ---------------------

% Overall evaluation: 1 (weak accept)

% ----------- Overall evaluation -----------

% This paper designs a distributed market for outsourcing computational resources. Compared to the traditional approaches, which are based on centralized management and volunteered resource sharing, the proposed system operates in a distributed and trustless manner. The authors develop smart contracts to enforce participants behaving honestly in the trading process. However, the actors may play this protocol in a few ways.

% 1) In section III-C, it mentions “The security deposit is a function of the maximum value of the posted offer, i.e., the maximum amount that the JC may pay or the RP may charge.” This means that JC may force a high security deposit on RP by raising the payment in the job offer.
% 1a) So what? If the RP does not have the funds, it will not be matched. If it does, then it will get a large payment. Either way, it's not a problem
% 2) A JC may devise a biased non-deterministic problem to play the protocol. For example, JC can post a non-deterministic question that answers YES with 10\% and NO with 90\%. If it gets NO from the RP, it will accept the result and pay the RP. If it gets YES, it will ask for mediation. Since the mediator will execute the problem twice, it has 0.9*0.9=81\% chance get two NOs and result in punishing the RP. \ise{covered by analysis}

% In addition, there are a few concepts mentioned in the paper that the authors may want to elaborate or unsophisticated. Below are examples of such concepts.
% 1) “penalty\_rate” is used in section III-C and the authors seem to forget explaining it in section IV. \ise{in section IV.F}
% 2) “capacity” is introduced in section III-A but never used in the rest of the paper. \ise{removed because doesn't belong in workflow. Use other language is solver section, or smart contract potentially if required}

% Besides, the author may want to split Figure. 2 (the entire workflow chart) by steps or by function calls. The current figure is hard to read. \ise{add curly braces.}


% ----------------------- REVIEW 3 ---------------------

% Overall evaluation: 1 (weak accept)

% ----------- Overall evaluation -----------

% This paper presented MODICUM, which is a decentralized platform for outsourcing computation. This platform can harness the untapped computational resources from the IOT devices. The authors provide analytic results proving that MODICUM deters misbehavior. 

% The authors claim that MODICUM is a decentralized platform, so it is not reasonable to assume that Mediators always act honestly. There should be punishment rules for the malicious mediators in case the mediators are in collusion with RPs or JCs. Although the malicious mediators could be removed, he can still get profit before that.

% To run the distributed ledger, if the main Ethereum chain was not used, full nodes should store all the data and run a consensus algorithm (PoW), which consume computing and storage resources. 

% Now the problem is: who will be the full nodes? To make the platform decentralized, it seems that the RPs and JCs should be full nodes. But I do not think the INCENTIVES are enough for RPs and JCs to be the full nodes of the blockchain. If the main Ethereum chain is used, the efficiency of the platform could be dragged down because the tps of Ethereum is only about 15.

% (a) - Malicious mediators: We need to discuss this in more detail and perhaps provide an outline of incentive analysis.

==> seq.tex <==
\iffalse
\begin{figure*} [!t]
\centering
\begin{tikzpicture}[x=5.65cm, y=-0.063cm, semithick, font=\small,
Event/.style={blue, dashed}]
\def\posJC{0}
\def\posSolver{0.5}
\def\posPlatform{1}
\def\posDirectory{1.5}
\def\posRP{2}
\def\posM{2.5}

\foreach \name/\pos in {JobCreator/\posJC, ResourceProvider/\posRP, \platform/\posPlatform, Solver/\posSolver, Directory/\posDirectory, Mediator/\posM} {
  \draw (\pos, 0) -- (\pos, 230);
  \node [draw, fill=white, rounded corners=0.1cm] at (\pos, 0) {\name};
}
\newcounter{seqTime}
\setcounter{seqTime}{0}
\foreach \action/\from/\to/\style/\delta in {
  {registerMediator/\posM/\posPlatform/solid/15},
  {MediatorRegistered/\posPlatform/\posSolver/Event/7},
  {MediatorRegistered/\posPlatform/\posJC/Event/7},
  {MediatorRegistered/\posPlatform/\posRP/Event/0},
  {registerJobCreator/\posJC/\posPlatform/solid/7},
  {registerResourceProvider/\posRP/\posPlatform/solid/0},
  {ResourceProviderRegistered/\posPlatform/\posSolver/Event/7},
  {JobCreatorRegistered/\posPlatform/\posSolver/Event/7},
  {jobCreatorAddTrustedMediator/\posJC/\posPlatform/solid/7},
  {resourceProviderAddTrustedMediator/\posRP/\posPlatform/solid/0},
  {ResourceProviderAddedTrustedMediator/\posPlatform/\posSolver/Event/7},
  {JobCreatorAddedTrustedMediator/\posPlatform/\posSolver/Event/7},
  {uploadJob/\posJC/\posDirectory/solid/7},
  {postJobOffer/\posJC/\posPlatform/solid/7},
  {postResOffer/\posRP/\posPlatform/solid/0},
  {ResourceOfferPosted/\posPlatform/\posSolver/Event/7},
  {JobOfferPosted/\posPlatform/\posSolver/Event/7},
  {JobOfferPosted/\posPlatform/\posRP/Event/0},
  {cancelJobOffer/\posJC/\posPlatform/dotted/7},
  {cancelResOffer/\posRP/\posPlatform/dotted/0},
  {JobOfferCanceled/\posPlatform/\posSolver/Event/7},
  {ResourceOfferCanceled/\posPlatform/\posSolver/Event/7},
  {postMatch/\posSolver/\posPlatform/solid/7},
  {Matched/\posPlatform/\posRP/Event/7},
  {Matched/\posPlatform/\posJC/Event/0},
  {getJobImage/\posRP/\posDirectory/solid/7},
  {uploadResult/\posRP/\posDirectory/solid/7},
  {postResult/\posRP/\posPlatform/solid/7},
  {ResultPosted/\posPlatform/\posJC/Event/7},
  {timeout/\posJC/\posPlatform/dotted/7},
  {getResult/\posJC/\posDirectory/solid/7},
  {acceptResult/\posJC/\posPlatform/solid/7},
  {MatchClosed/\posPlatform/\posJC/Event/7},
  {MatchClosed/\posPlatform/\posRP/Event/0},
  {rejectResult/\posJC/\posPlatform/red/7},
  {JobAssignedForMediation/\posPlatform/\posM/Event/7},
  {postMediationResult/\posM/\posPlatform/red/7},
  {MediationResultPosted/\posPlatform/\posJC/Event/7},
  {MatchClosed/\posPlatform/\posJC/Event/7},
  {MatchClosed/\posPlatform/\posRP/Event/0}%
} {
  \addtocounter{seqTime}{\delta}
  \draw [->, >=stealth, shorten <=0.05cm, shorten >=0.05cm, \style] (\from, \value{seqTime}) -- (\to, \value{seqTime}) node [midway, above, align=center, text width={abs(\to - \from) * 5.1cm}, fill=white, fill opacity=0.67, text opacity=1] {\footnotesize\texttt{\scriptsize\action}};
}
\end{tikzpicture}
\caption{Sequence diagram showing the outsourcing of a single job. Black arrows are function calls to the smart contract. Blue dashed lines are events emitted by the smart contract. Black dotted lines are optional function calls. Red lines are optional calls that are required in case of disagreement between RP and JC.}
\label{fig:seqdiag}
\end{figure*}
\fi
% \textcolor{red}{mention solid black arrows as well}

==> tables/collusion-outcome-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\caption{Outcomes of Collusion scenarios. \textcolor{red}{not sure how to close the cell gaps or prevent the gray from extending on the right side.}}
\label{tab:collusion}
\begin{tabular}[\textwidth]{@{}p{0.07\textwidth}p{0.15\textwidth}p{0.25\textwidth}p{0.25\textwidth}p{0.2\textwidth}@{}}
\toprule
 &
  Solver &
  Mediator &
  Directory &
  Resource Provider \\ \midrule
Job Creator &
  Intentional and~harmless. &
  Honest RP removes the Mediator and Directory from its trusted list. Thus a mediator can only launch this attack once per RP. Additionally the Directory removes the Mediator from its trusted list. &
  Honest RP removes the Mediator and Directory from its trusted list. Thus a Directory can only launch this attack once per RP. Additionally the Mediator removes the Directory from its trusted list. &
  JC colludes with RP. There is no benefit to this collusion. It results in a  loss \\
\hline Resource Provider &
  Intentional and~harmless. &
  Honest JC removes the Mediator, and Directory from its trusted list.  Thus a mediator can only launch this attack once per JC. Additionally the Directory removes the Mediator from its trusted list. &
  Honest JC removes the Mediator and Directory from its trusted list. Thus a Directory can only launch this attack once per RP. Additionally the Mediator removes the Directory from its trusted list. &
  \cellcolor[HTML]{C0C0C0} \\
\hline Directory &
  No apparent benefit. &
  JC/RP will have the same response as if the RP/JC were colluding with the Directory or Mediator. &
  \cellcolor[HTML]{C0C0C0} &
  \cellcolor[HTML]{C0C0C0} \\
\hline Mediator &
  Potential unfairness;  however not a concern since the JC or RP can act as Solver. &
  \cellcolor[HTML]{C0C0C0} &
  \cellcolor[HTML]{C0C0C0} &
  \cellcolor[HTML]{C0C0C0} \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/collusion-table.tex <==

\begin{table*}[]
% \small
\footnotesize
\caption{\revision{Outcomes of Collusion scenarios. }}
\label{tab:collusion}
\begin{tabular}{@{}p{0.07\textwidth}p{0.25\textwidth}p{0.3\textwidth}p{0.25\textwidth}p{0.12\textwidth}@{}}
\hline
                  & Solver                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     & Mediator                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          & Directory                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 & Resource Provider                                                                 \\ \hline
Job Creator       & JC colludes with or acts as a Solver. Since the offers are public the JC/solver will match its own offers with the resource offer with the lowest unit price. This means the RP with the lowest offer will be matched first. Also since the resource offer includes the minimum amount it requires to rent out resources, proposed trades that offer less than the required amount will be rejected by the contract. So the JC cannot force the RP to do work for less than RP specified in its offer. There is no harm in this collusion. & JC colludes with Mediator. Regardless of what the RP does the JC rejects the result and the Mediator rules in favor of the JC. An honest RP will know that it attempted to execute the job correctly, and may make one of three assumptions. 1) The job was non-deterministic and the Mediator was tricked, 2) The Mediator is faulty (this includes colluding) 3) The Directory is faulty. Rather than trying to differentiate the cases the RP simply removes the Mediator and Directory from its trusted list. Thus a mediator can only launch this attack once per RP. Additionally the Directory removes the Mediator from its trusted list. & JC colludes with Directory. The Directory can modify the job, the result, claim job is not present, or be unavailable. Modification is detectable by the Mediator and provides no benefit. Claiming the job is not present or being unavailable to the RP are effectively the same, the Mediator can be forced to rule in favor of the JC. In this case the RP removes the Mediator and Directory from its trusted list. Thus a Directory can only launch this attack once per RP. Additionally the Mediator removes the Directory from its trusted list. & JC colludes with RP. There is no benefit to this collusion. It results in a  loss \\
\hline
Resource Provider & RP colludes with or acts as a Solver. Since the offers are public the RP/solver will match its own offers with the Job offer with the highest unit price. This means the JC with the highest offer will be matched first. Also since the job offer includes the maximum amount the JC is willing to pay for resources and proposed match that exceeds that will be rejected by the contract. So the RP cannot force the JC to pay more than it specifies in the offer. There is no harm in this collusion.                                 & RP colludes with Mediator. The RP does not perform the computation and the JC will request mediation and the Mediator rules in favor of the RP. The JC knows that the result is incorrect and that there was collusion between at least two of \{RP, Mediator, Directory\}. The JC removes the Mediator, and Directory from its trusted list.  Thus a mediator can only launch this attack once per JC. Additionally the Directory removes the Mediator from its trusted list.                                                                                                                                                                    &       RP colludes with Directory. The Directory can modify the result, claim result is not present, or be unavailable. Modification is detectable by the Mediator and provides no benefit. Claiming the result is not present or being unavailable to the JC are effectively the same, the Mediator can be forced to rule in favor of the RP. In this case the JC removes the Mediator and Directory from its trusted list. Thus a Directory can only launch this attack once per RP. Additionally the Mediator removes the Directory from its trusted list.                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    &                                                                                   \\
\hline
Directory         & \revision{I can't think of anything for this one}                                                                                                                                                                                                                                                                                                                                                                                                                                                                         & Directory Colludes with Mediator. The Directory can ensure that the JC will request Mediation by manipulating the job or the result. Depending on how the Mediator rules, the JC/RP will have the same response as if the RP/JC were colluding with the Directory or Mediator.                                                                                                                                                                                                                                                                                                                                                                    &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           &                                                                                   \\
\hline
Mediator          & Mediator colludes with Solver. The solver could prioritize trades that include the specific Mediator, and further prioritize JC and RP with history of requiring mediation. This could result in unfairness i.e., some jobs are never accepted. This is not a concern however since the JC or RP can act as Solver if this appears to be a problem.                                                                                                                                                                                        &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   &                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           &                                                                                   \\ \hline
\end{tabular}
\end{table*}

==> tables/gas-table.tex <==
% \ifFull{
\begin{table}
\caption{Gas cost for each platform function call, measured upon receipt of event emitted by that function. gasEstimate is the value returned when calling the eth\_estimateGas method}
\label{tab:gas_cost}
\begin{tabular}{@{}llll@{}}
\toprule
Function                 & mean     & std.dev. & gasEstimate \\ \midrule
setPenaltyRate           & 4.34E+04 & 0.00E+00 & 2.21E+04    \\
setReactionDeadline      & 4.31E+04 & 0.00E+00 & 2.16E+04    \\
acceptResult             & 1.40E+05 & 6.47E+04 & 6.29E+04    \\
postResult               & 1.91E+05 & 1.60E+04 & 2.25E+05    \\
postMatch                & 1.35E+05 & 1.70E+03 & 1.27E+05    \\
postJobOfferPartOne      & 2.36E+05 & 4.59E+03 & 2.28E+05    \\
postJobOfferPartTwo      & 2.16E+05 & 0.00E+00 & 2.27E+05    \\
postResOffer             & 2.42E+05 & 2.16E+03 & 2.32E+05    \\
registerMediator         & 1.37E+05 & 0.00E+00 & 8.51E+04    \\
registerResourceProvider & 8.12E+04 & 0.00E+00 & 2.54E+04    \\
resourceProviderAddTM    & 6.50E+04 & 0.00E+00 & 4.23E+04    \\
registerJobCreator       & 3.40E+04 & 0.00E+00 & 3.20E+03    \\
jobCreatorAddTM          & 6.53E+04 & 0.00E+00 & 4.26E+04    \\
postMediationResult      & 1.87E+05 & 1.56E+04 & 2.40E+05    \\
rejectResult             & 5.39E+04 & 9.90E+00 & 4.71E+04    \\
nominal cost             & 5.92E+05 &          &             \\ \bottomrule
\end{tabular}
\end{table}
% }
% \else
% {
% \begin{table}[h]
%     \caption{Gas cost for each platform function call, measured upon receipt of event emitted by that function. gasEstimate is the value returned when calling the eth\_estimateGas method}
%     \centering
%     {\tabcolsep1.4mm%
%     \csvreader[no head,before reading=\sisetup{round-mode=places,round-precision=2,round-integer-to-decimal}
%         \begin{adjustbox}{max width=\columnwidth},
% after reading=\end{adjustbox},
%      tabular=|l|*{3}{r}|,
%      nohead,column count=4,
%      table head=\hline,
%     late after first line=\\\hline,
%     table foot=\hline]{data/gas/gas.csv}%
%     {}%
%     {\csvlinetotablerow}
%     }
%     \label{tab:gas_cost}
% \end{table}{}
% }
% \fi

==> tables/payoffs.tex <==
% https://www.tablesgenerator.com/#
\begin{table}[]
\caption{Payoffs for each game outcome. Mediator receives $\pi_{m}+\pi_{a}$ for outcomes $o_1$}
\label{tab:payoffs}
\begin{tabular}{@{}cllll@{}}
\toprule
\multicolumn{1}{l}{Outcome} & Party & \begin{tabular}[c]{@{}l@{}}Contract\\ Payoff\end{tabular} & \begin{tabular}[c]{@{}l@{}}External\\ Payoff\end{tabular} & Total         \\ \hline
\multirow{2}{*}{$o_1$}      & RP    & $r$                                                       & $-C_d$                                                    & $r - C_d$     \\
                            & JC    & $-D$                                                      & $-C_r - C_v$                                              & $-D-C_r-C_v$  \\
                            \addlinespace[5pt]
\multirow{2}{*}{$o_2$}      & RP    & $-D$                                                      & $-C_d$                                                    & $-D-C_d$      \\
                            & JC    & $r$                                                       & $-C_r-C_v$                                                & $r-C_r- C_v$  \\
                            \addlinespace[5pt]
\multirow{2}{*}{$o_3$}      & RP    & $\pi$                                                     & $-C_d$                                                    & $\pi - C_d$   \\
                            & JC    & $-\pi$                                                    & 0                                                         & $-\pi$        \\
                            \addlinespace[5pt]
\multirow{2}{*}{$o_4$}      & RP    & $\pi$                                                     & $-C_e$                                                    & $\pi - C_e$   \\
                            & JC    & $-\pi$                                                    & $B$                                                       & $B-\pi$       \\
                            \addlinespace[5pt]
\multirow{2}{*}{$o_5$}      & RP    & $\pi$                                                     & $-C_e$                                                    & $\pi - C_e$   \\
                            & JC    & $-\pi$                                                    & $B-C_v$                                                   & $B-\pi-C_v$   \\
                            \addlinespace[5pt]
\multirow{2}{*}{$o_6$}      & RP    & $r$                                                       & $-C_e$                                                    & $r - C_e$     \\
                            & JC    & $-D$                                                      & $B-C_r-C_v$                                               & $B-D-C_r-C_v$ \\
                            \addlinespace[5pt]
\multirow{2}{*}{$o_7$}      & RP    & $-D$                                                      & $-C_e$                                                    & $-D-C_e$      \\
                            & JC    & $r$                                                       & $B-C_r-C_v$                                               & $B+r-C_r-C_v$ \\ 
\bottomrule
\end{tabular}
\end{table}
